Initialization Matters for Adversarial Transfer Learning

With the prevalence of the Pretraining-Finetuning paradigm in transfer learning, the robustness of downstream tasks has become a critical concern. In this work, we delve into adversarial robustness in transfer learning and reveal the critical role of initialization, including both the pretrained model and the linear head. First, we discover the necessity of an adversarially robust pretrained model. Specifically, we reveal that with a standard pretrained model, Parameter-Efficient Finetuning (PEFT) methods either fail to be adversarially robust or continue to exhibit significantly degraded adversarial robustness on downstream tasks, even with adversarial training during finetuning. Leveraging a robust pretrained model, surprisingly, we observe that a simple linear probing can outperform full finetuning and other PEFT methods with random initialization on certain datasets. We further identify that linear probing excels in preserving robustness from the robust pretraining. Based on this, we propose Robust Linear Initialization (RoLI) for adversarial finetuning, which initializes the linear head with the weights obtained by adversarial linear probing to maximally inherit the robustness from pretraining. Across five different image classification datasets, we demonstrate the effectiveness of RoLI and achieve new state-of-the-art results. Our code is available at \url{https://github.com/DongXzz/RoLI}.

==> sec/5_methods.tex <==
\section{Initialization Matters For Finetuning}
\label{sec:methods}
In the previous section, we understand the necessity of initializing a model with an adversarially robust pretrained model. 
% Given an adversarially robust pretraining, we want to ask: \textit{What method should we use in adversarial transfer learning?}
We now ask: \emph{given a robust pretrained model, what matters for adversarial finetuning?}

 %-------------------------------------------------------------------------

\begin{table}[]
\small
\setlength\tabcolsep{0.3cm}
\centering
\begin{tabular}{l|cc|cc}
\toprule
\multirow{2}{*}{Methods} & \multicolumn{2}{c}{ViT} & \multicolumn{2}{|c}{Swin} \\
                         & Clean      & PGD        & Clean       & PGD        \\
\midrule
RanLI - Full-FT          & 80.17      & 44.15      & 85.19       & 54.13      \\
RanLI - Adapter          & 83.14      & 49.57      & 85.24       & 54.22      \\
RanLI - LoRa             & 82.63      & 50.72      & 83.52       & 53.57     \\
RanLI - Bias             & 82.69      & 50.07      & 84.88       & 54.69      \\
RanLI - VPT              & 82.09      & 50.52      & 84.99       & 55.23      \\
RanLI - Linear           & 81.89      & 42.02      & 82.98       & 45.89      \\
\bottomrule
\end{tabular}
\caption{\textbf{PEFT methods, excluding Linear, demonstrate strong performance on average across CIFAR-10 and Caltech-256 datasets.} With adversarial finetuning, PEFT methods outperform Full-FT and Linear with random linear initialization.}
\label{tab:RanLI}
\end{table}


\subsection{Random Linear Initialization}\label{sec:ranli}

To answer this question, we first evaluate the adversarial robustness of six adversarial finetuning techniques. To adapt the robust pretrained model to the downstream tasks, we initialize the linear head with Random Linear Initialization (RanLI) following~\cite{artl}. We perform adversarial finetuning across two model architectures, e.g., ViT and Swin, on the CIFAR-10 and Caltech-256 datasets. Additional details regarding the training process can be found in \cref{subsec:details} and in the supplementary materials. 

As shown in \cref{tab:RanLI}, PEFT methods except Linear consistently demonstrate strong average results with adversarial finetuning. In particular, LoRA achieves the highest average robustness at 50.72\% for ViT, while VPT performs exceptionally well with 55.23\% on Swin.

% We conduct experiments using six popular finetuning methods with random linear initialization. Here, random linear initialization refers to initializing the linear head that maps features to the output space randomly. Our model training involves two architectures, namely ViT and Swin, on the CIFAR-10 and Caltech-256 datasets. Additional details regarding the training process can be found in \cref{subsec:details} and in the supplementary materials.

% \cref{tab:RanLI} illustrates that, except for linear probing, PEFT methods consistently demonstrate strong average results with adversarial finetuning. Notably, LoRA achieves the highest average robustness at 50.72\% for ViT, while VPT performs exceptionally well with 55.23\% on Swin.

Looking more closely at the performance on each individual dataset in \cref{fig:confounder}, we observe that adversarial linear probing achieves the strongest robustness on Caltech256. 
% 
% However, when evaluating individual dataset performance in \cref{fig:confounder}, we observe that linear probing excels other methods when applied to the Caltech256 but encounters challenges on the CIFAR-10. 
This is rather surprising, given that linear probing has the lowest computational cost compared to others and never outperforms other finetuning methods on any single dataset in standard transfer learning~\cite {vpt,glora,adaptformer}.

\subsection{Why does Adversarial Linear Probing Work?}\label{sec:why}
To understand the remarkable robustness achieved by adversarial linear probing, we then ask: \emph{what contributes to adversarial robustness on the downstream tasks given a robust pretrained model?} We hypothesize that there are two confounding factors: 1) the robustness inherited from pretrained models, and 2) the robustness achieved by adversarial finetuning. To validate our hypothesis, we conduct a comparative analysis of adversarial robustness in downstream tasks while using standard finetuning versus adversarial finetuning, given the same robust pretrained model. 

\vspace{-3mm}
\paragraph{Robustness Inherited from Pretrained Models.} 
% Looking at Standard finetuning shown in Blue color in Figure~\ref{fig:confounder}, we aim to investigate if adversarial robustness from downstream tasks can inherit from robust pretrained model, we use the adversarial robustness on the downstream tasks while performing standard finetuning given a robust pretrained model. 
In this section, we focus on \emph{standard finetuning} as it does not bring in additional adversarial robustness to downstream tasks. Therefore, the adversarial robustness achieved during {standard finetuning}  primarily arises from the robust pretrained model, representing the capability of each method to preserve robustness from the pretrained model. As shown in \cref{fig:confounder}, all standard finetuning methods (colored in blue) achieve non-zero robustness under PGD-10 attacks. This supports our hypothesis that robustness inherited from the pretrained model contributes to the robustness in downstream tasks. In addition, linear probing significantly outperforms all other standard finetuning methods in preserving robustness from the pretrained model. For example, linear probing exhibits significantly stronger robustness (at least 20\% higher) compared to other methods while maintaining similar accuracy on Caltech-256. We explain this as linear probing avoids distorting the robust features inherited from the pretrained model by only updating the linear head. However, on CIFAR-10, linear probing does not exhibit a significant advantage over robustness and displays lower clean accuracy compared to others. This is likely due to its limited capability to adapt features from the pretrained source domain to the downstream target domain.
\vspace{-3mm}
\paragraph{Robustness Achieved by Adversarial Finetuning.} By comparing adversarial robustness achieved by standard finetuning (colored in blue) and adversarial finetuning (colored in red) in \cref{fig:confounder}, we can see the extra robustness gain achieved by adversarial training during the finetuning stage. Except for Linear, adversarial finetuning contributes a significant portion of their robustness to the final robustness. For example, Full-FT on Swin, achieving a 99\% final robustness on Caltech-256 through adversarial finetuning. Even VPT, which has the fewest tunable parameters after Linear, demonstrates a 78\% final robustness from adversarial finetuning. On the contrary, Linear only achieved a final robustness of 13\% from this stage, with the primal robustness originating from the pretraining model. 
 % adversarial linear probing excels in inheriting robustness from pretrained model, whereas other methods primarily obtain their robustness from adversarial training during finetuning stage. 

Taken together, we validate our hypothesis that both robustness inherited from the pretrained model and achieved through adversarial finetuning contribute to adversarial robustness on downstream tasks. In addition, we conclude that the exceptional robustness exhibited by adversarial linear probing is mainly because linear probing excels in preserving robustness from pretrained models compared to others, which primarily obtain their robustness from adversarial training during finetuning stage. 

\subsection{Transferred Robustness Correlates with Transferred Accuracy.}
\label{subsec:transferred acc and rob}
As we have seen in \cref{fig:confounder}, adversarial linear probing achieves the highest adversarial robustness on Caltech-256 but falls far behind other methods on CIFAR-10. This performance discrepancy across different datasets raises a question: \emph{how can we estimate if adversarial linear probing achieves the best robustness?} Based on our analysis in \cref{sec:why}, where the robustness of adversarial linear probing primarily arises from preserving the robustness in the pretrained model, we hypothesize that the transferred robustness of adversarial linear probing is highly correlated with the transferred accuracy of standard linear probing. This suggests that if standard linear probing successfully adapts the features from the pretrained source domain to the downstream target domain, adversarial linear probing will similarly preserve the robustness in the pretrained model. 

\begin{table*}[]
\small
\centering
\setlength{\tabcolsep}{7.1pt}
\begin{tabular}{l|cccccccccc|cc}
\toprule 
\multirow{2}{*}{Methods} & \multicolumn{2}{c}{CIFAR-10} 
& \multicolumn{2}{c}{CIFAR-100} & \multicolumn{2}{c}{Caltech-256} & \multicolumn{2}{c}{CUB200} & \multicolumn{2}{c}{Stanford Dogs} & \multicolumn{2}{|c}{Average} \\
% \cmidrule{2-3} \cmidrule{4-5}
% & \cline{2-3} & \cline{4-5} &  \cline{6-7} &  \cline{8-9}\\
                         & Clean        & PGD        & Clean         & PGD        & Clean         & PGD         & Clean        & PGD       & Clean           & PGD          & Clean        & PGD       \\
                         \midrule
TWINS-AT~\cite{twins} & 91.24 & 52.73 & 70.72 & 31.08 & 76.86 & 48.40 & 68.09 & 29.24 & 64.98 & 20.58 & 74.38 & 36.41 \\
AutoLoRa~\cite{autolora} & 86.93 & 57.16 & 66.20 & 35.25 & 69.85 & 47.82 & 62.78 & 31.07 & 62.33 & 25.32 & 69.62 & 39.32 \\
\midrule
RanLI - Full-FT    & 93.02 & 59.12  & 74.36 & 35.62  & 77.35 & 49.13  & 70.83 & 31.55  & 65.85 & 24.79  & 76.28 & 40.04  \\
RanLI - Adapter    & 90.23 & 55.70  & 71.57 & 34.74  & 80.24 & 52.73  & 59.67 & 26.73  & 87.98 & 42.24  & 77.94 & 42.43  \\
RanLI - LoRA       & 90.02 & 56.88  & 71.98 & 34.83  & 77.02 & 50.25  & 64.74 & 29.65  & 84.63 & 39.24  & 77.68 & 42.17  \\
RanLI - Bias       & 90.25 & 56.94  & 71.50  & 36.72  & 79.50 & 52.43  & 66.69 & 29.88  & 87.41 & 42.75  & 79.07 & 43.74  \\
RanLI - VPT        & 90.24 & 57.38  & 72.37 & 35.60   & 79.74 & 53.07  & 61.94 & 26.46  & 86.34 & 43.10  & 78.13 & 43.12  \\
RanLI - Linear     & 84.16 & 37.30  & 67.65 & 25.46  & 81.79 & 54.47  & 69.88 & 24.56  & 91.55 & 45.45  & 79.01 & 37.45  \\
\midrule
RoLI - Full-FT     & \textbf{94.18} & \textbf{60.85}  & \textbf{76.25} & \textbf{37.38}  & \textbf{83.78} & \textbf{55.42}  & \textbf{74.28} & \textbf{32.03}  & 91.55 & 45.57  & \textbf{84.01} & \textbf{46.25}  \\
RoLI - Adapter     & 90.31 & 55.69  & 71.75 & 34.33  & 81.74 & 54.32  & 64.20 & 25.22  & \textbf{92.02} & 47.12  & 80.00 & 43.34  \\
RoLI - LoRA        & 92.23 & 58.62  & 72.87 & 35.18  & 81.79 & 54.50  & 68.88 & 26.77  & 91.20 & 46.76  & 81.39 & 44.37  \\
RoLI - Bias        & 91.83 & 58.39  & 72.17 & 35.17  & 81.78 & 54.49  & 68.14 & 25.70  & 91.52 & \textbf{47.27}  & 81.09 & 44.20  \\
\bottomrule        
\end{tabular}
\caption{\textbf{RoLI significantly improves the performance and achieves SOTA across five image classification tasks.} 
% With random linear initialization~(RanLI), the PEFT methods demonstrate relatively good average performance, with Bias achieving the highest average performance. 
Robust Linear Initialization~(RoLI) enhances robustness by 3.88\% and clean accuracy by 2.44\% on average compared to Random Initialization (RanLI). Notably, RoLI - Full-FT achieves the best overall performance, with an accuracy of 84.01\% and 46.25\% robustness.}
\label{tab:benchmark}
\end{table*}

% Since linear probing will not distort the robust features in the pretrained model, we conjecture that the crucial factor influencing the performance of robust transfer learning in linear probing lies in its capacity to adapt effectively to the targeted domain. 
% To evaluate the feature adaptation capability for linear probing, 
To validate this, we define \textbf{transferred accuracy} of standard linear probing ($\text{acc}^T_{std}$) and \textbf{transferred robustness} of adversarial linear probing ($\text{rob}^T_{adv}$) as follows, using full finetune as a baseline to normalize the performance across different datasets:

\begin{equation}
  \text{acc}^T_{std} = \frac{\text{acc}(LP_{std}) - \text{acc}(FT_{std})}{\text{acc}(FT_{std})}
  \label{eq:transferred accuracy}
\end{equation}
\begin{equation}
  \text{rob}^T_{adv} = \frac{\text{rob}(LP_{adv}) - \text{rob}(FT_{adv})}{\text{rob}(FT_{adv})}
  \label{eq:transferred robustness}
\end{equation}
where $\text{acc}(\cdot)$ and $\text{rob}(\cdot)$ denote the accuracy and robustness of each method, respectively. $FT_{std}$ and $LP_{std}$ represent standard full finetune and standard linear probing whereas $FT_{adv}$ and $LP_{adv}$ stand for their respective adversarial counterparts. We trained 51 models with different hyper-parameter settings across five datasets and present transferred accuracy and robustness in \cref{fig:indicator}.

\begin{figure}[t]
  \centering
   \includegraphics[width=0.9\linewidth]{sec/figs/indicator_v4.pdf}
\vspace{-3mm}
   \caption{Transferred robustness of adversarial linear probing strongly correlates with transferred accuracy of standard linear probing.}
   \label{fig:indicator}
   \vspace{-3mm}
\end{figure}

In \cref{fig:indicator}, the transferred robustness of adversarial linear probing is strongly correlated with the transferred accuracy of standard linear probing, with a high Pearson correlation coefficient (0.896). When the transferred accuracy approaches or surpasses 0, the transferred robustness becomes positive, indicating the improved performance of adversarial linear probing over adversarial fully finetuning. This strong correlation validates our hypothesis that if standard linear probing successfully adapts features from the pretrained to the target domain, its adversarial counterpart is capable of effectively achieving adversarial robustness on downstream tasks.
\vspace{-1mm}
\subsection{Robust Linear Initialization (RoLI)}
\label{subsec:details}
% \paragraph{Robust Linear Initialization (RoLI).} 
Based on our observation that linear probing can outperform other methods when it effectively adapts features to the target domain, we propose Robust Linear Initialization (denoted as RoLI) for adversarial finetuning. Specifically, we initialize the linear head of a robust pretrained model with weights obtained through adversarial linear probing instead of random initialization. Then, we perform adversarial finetuning, using either full finetune or PEFT methods. Since adversarial linear probing excels in preserving robustness from a pretrained model, RoLI provides a more robust initialization for subsequent adversarial finetuning, maximizing the robustness inherited from a robust pretrained model. In addition, the following adversarial finetuning can further enhance robustness by introducing additional robustness through adversarial training. 
%
In the following sections, we will evaluate the effectiveness of RoLI applied to four different adversarial finetuning methods across five different datasets and demonstrate it achieves new state-of-the-art robustness in adversarial transfer learning.

% ; on the other hand, even if adversarial linear probing Given that linear probing may exhibit limited performance on some datasets due to its restricted feature adaptation capability, the subsequent finetuning methods, which has strong feature adaptation capabilities, can further enhance the final performance. We evaluate our RoLI as follows:
\vspace{-2mm}
\paragraph{Datasets.} In our experiments, we use five datasets: CIFAR-10~\cite{cifar}, CIFAR-100~\cite{cifar}, Caltech-256~\cite{caltech}, Caltech-UCSD Birds-200-2011 (CUB200)~\cite{cub}, and Stanford Dogs~\cite{stanforddogs}. 
% For CIFAR-10 and CIFAR-100, we follow the official train-validation-test splits. Since there are no official train-validation-test splits available for other datasets, we randomly sample images to create training and validation sets, 
% % However, as official splits are not available for the other datasets, we randomly sample the training and validation sets, 
% with additional details provided in the supplementary material. 
For low-resolution image datasets like CIFAR10 and CIFAR100, we resize the image to match the model input shape.  For high-resolution image datasets, we apply random resizing and cropping in training and center crop in testing. It's important to note that we integrate the resizing and normalization process directly into the model since the attacker does not have access to pre-processed images. Additional details are provided in the supplementary material.


\paragraph{Methods.} We provide the results from TWINS-AT~\cite{twins} AutoLoRa~\cite{autolora} as baselines. We proceed to assess six finetuning techniques introduced in \cref{subsec:PEFTs} with random initialization. We use Swin Transformer~\cite{swin} as a backbone architecture for our experiments, whereas TWINS and AutoLoRa use ResNet50~\cite{resnet}. We apply RoLI to Full-FT, Bias, Adapter, and LoRa. We initialize the newly introduced modules in Adapter and LoRA with zero to ensure that they start with robust linear probing without distorting the robust features preserved in the pretrained model. 
% the starting point aligns with the endpoint of linear probing, preserving robust features before finetuning 
% \footnote{We do not implement RoLI-Prompt as zero initialization would still distort the features due to the attention module}. 
\paragraph{Training Details.} 
% We use the same optimizer, AdamW~\cite{adamw}, and scheduler, a cosine scheduler with warm-up, for all finetuning methods. 
We use the same optimizer, AdamW~\cite{adamw}, and a cosine scheduler with warm-up for all finetuning methods. To determine the optimal learning rate and weight decay values, we conduct a grid search, and the ranges of hyper-parameters along with the optimal combinations can be found in the supplementary material. We keep method-specific hyper-parameters constant across all datasets. For instance, we set the prompt length to 10 for the VPT method. To avoid adversarial overfitting~\cite{overfitadv}, we apply early stopping with the epoch that has the best performance on the validation set. During adversarial finetuning, we utilize the PGD-7 attack with ${\varepsilon} = 8/255$ and a step size of ${\alpha}= 2/255$. When reporting test accuracy and robustness, we evaluate the models under a PGD-10 attack with ${\varepsilon} = 8/255$.
% \vspace{-3mm}

\begin{figure}[t]
\vspace{-4mm}
  \centering
   \includegraphics[width=0.85\linewidth, ,height=0.62\linewidth]{sec/figs/speed_v1.pdf}
   \caption{\textbf{Trade-off between speed and robustness.} We conduct the speed test on Stanford Dogs with random linear initialization~(RanLI), logistic regression linear initialization~(RegLI), standard linear initialization~(StdLI), and robust linear initialization~(RoLI). RoLI achieves the best performance at the cost of increased training time. Meanwhile, both RegLI and StdLI can improve their performance without incurring substantial time costs.}
   \label{fig:speed}
   % \vspace{-3.5mm}
\end{figure}

\paragraph{Experimental Results.} Looking at Random Initialization (RanLI) in \cref{tab:benchmark}, the same trend holds as in \cref{sec:ranli}: 1) PEFT methods except linear probing exhibit strong average results across five different datasets, with Bias achieving the best performance (79.25\% accuracy and 43.58\% robustness). 2) Linear probing achieves the highest robustness on Caltech256 and Stanford Dogs, although it falls behind others on the remaining three datasets. 
% This variability in performance contributes to relatively low average performance for linear probing.

Compared to RandLI, we can observe from \cref{tab:benchmark} that RoLI significantly enhances the robustness on Caltech256 and Stanford Dogs for all finetuning methods. In particular, RoLI - Full-FT achieves a robustness improvement of 6.29\% on Caltech256 and 20.78\% on Stanford Dogs. On other datasets where adversarial linear probing with RanLI does not outperform others, RoLI performs comparable or even better than RanLI. This strongly supports that a robust initialization of the linear head is critical in adversarial transfer learning. Lastly, our RoLI - Full-FT achieves the highest performance across five datasets and sets a new state-of-the-art benchmark.

% that require a strong feature adaptation, such as CIFAR-10 and CIFAR-100, RoLI can achieve a comparable or even better performance compared with RanLI. Finally, RoLI - Full-FT can achieve the highest performance across five datasets and set a new state-of-the-art benchmark.



==> sec/7_conclusion.tex <==
\section{Conclusion}
This paper systematically investigates how to achieve adversarial robustness in downstream tasks. We observe that PEFT methods either fail to be adversarially robust or exhibit significantly degraded adversarial robustness when initialized with a non-robust pretraining, highlighting the necessity of an adversarially robust pretraining. Given a robust pretrained model, we propose to use robust linear initialization~(RoLI) followed by adversarial full finetuning or PEFT methods to achieve the best performance. This is motivated by our understanding that adversarial linear probing maximally inherits the robustness from the pretraining and the following adversarial finetuning can adapt the features to the downstream tasks effectively. 
% Finally, we conduct a comprehensive evaluation of RoLI across five image classification tasks and demonstrate a stronger performance compared with random linear initialization. 
% 
We demonstrate that RoLI outperforms random linear initialization across five image classification tasks. We hope the insights from this study greatly advance research aimed at enhancing adversarial robustness in downstream tasks. Furthermore, we believe that these findings offer invaluable guidance for developing robust models in the real world.
% Additionally, we hope practitioners can acknowledge the necessity of robust pretraining to downstream robustness and encourage practitioners to pay more attention to large-scale adversarial robust models.

% I'll add the future work first
% move fig7 and fig8 same page
% move figure 5 to previous page

